Crowd counting via scale-adaptive convolutional neural network

The task of crowd counting is to automatically estimate the pedestrian number in crowd images. To cope with the scale and perspective changes that commonly exist in crowd images, state-of-the-art approaches employ multi-column CNN architectures to regress density maps of crowd images. Multiple columns have different receptive fields corresponding to pedestrians (heads) of different scales. We instead propose a scale-adaptive CNN (SaCNN) architecture with a backbone of fixed small receptive fields. We extract feature maps from multiple layers and adapt them to have the same output size; we combine them to produce the final density map. The number of people is computed by integrating the density map. We also introduce a relative count loss along with the density map loss to improve the network generalization on crowd scenes with few pedestrians, where most representative approaches perform poorly on. We conduct extensive experiments on the ShanghaiTech, UCF_CC_50 and WorldExpo datasets as well as a new dataset SmartCity that we collect for crowd scenes with few people. The results demonstrate significant improvements of SaCNN over the state-of-the-art.

==> tex/sec-overview.tex <==
\section{Overview}

==> tex/sec-relatedwork.tex <==
\section{Related work}
We categorize crowd counting methods as either 1) detection-based methods or 2) regression-based methods. We shall describe both categories below and compare representative works to our method.

\subsection{Detection-based methods}
These methods detect each individual in a crowd. Early works focus on video surveillance scenario so that the
motion and appearance cues can be utilized~\cite{viola2003ijcv,brostow2006cvpr,rabaud2006cvpr}.
Since pedestrian occlusions commonly occur in a dense crowd, part-detectors were employed to count pedestrian via human body parts~\cite{wang2011cvpr,wu2005iccv}. \cite{stewart2016cvpr} took advantage of a recurrent deep network to detect heads in crowd scenes. Notwithstanding their improvement, detection-based methods overall suffer severely in dense crowds with high occlusions among people.

\subsection{Regression-based methods}
These methods regress either a scalar value (pedestrian number) or a density map on various features extracted from crowd images. Earlier works use handcrafted features, like edge features~\cite{chan2008cvpr,chen2012bmvc,ryan2009dicta,regazzoni1996sp} and texture features~\cite{chen2012bmvc,idrees2013cvpr,marana1998sibgrapi}. Regression methods include linear~\cite{regazzoni1996sp,paragios2001cvpr}, ridge~\cite{chen2012bmvc} and Gaussian~\cite{chan2008cvpr} functions.
%They regress either a scalar value (pedestrian number)~\cite{chan2008cvpr,chan2009iccv,liu2015iccv,idrees2013cvpr} or a density map~\cite{chen2012bmvc,kong2005bmvc,lempitsky2010nips}.

Due to the use of strong CNN features, recent works on crowd counting have shown remarkable progress by regressing a density map of an image~\cite{zhang2015cvpr,zhang2016cvpr,sam2017arxiv,boominathan2016mm,onoro2016eccv}. %The ground truth in crowd counting is not just the number of people but also their locations.
A density map provide much more information than a scalar value, and CNN have been particularly good at solving problems ``locally" rather than ``globally".%, present works thus regress density maps~\cite{zhang2015cvpr,zhang2016cvpr,sam2017arxiv,boominathan2016mm}.
%They regress either a scalar value (pedestrian number) or a density map.
Crowd counting is casted as that of estimating a continuous density function whose integral over any image region gives the count of pedestrians within that region.
%It should be noted that  CNNs have been particularly good at solving problems ``locally" rather than ``globally".
\cite{zhang2015cvpr} designed a multi-task network to regress both density maps and crowd counts. They employed fully-connected layers to regress the absolute crowd count. %Because the two losses regarding the density map and crowd count are not in the same scale, they have to train the network in an alternating fashion by fixing one and training another.

\subsection{Comparison to our SaCNN}
\cite{zhang2016cvpr,sam2017arxiv,boominathan2016mm} utilized multi-column networks~\cite{ciregan2012cvpr} to deal with the variation of head scale in one image. Each column corresponds to different filter size. The large-sized filters make the whole network hard to train. The network is pretrained on each column first and finetuned together in the end~\cite{zhang2016cvpr}; whilst our SaCNN employs a single column with a single filter size which can be trained from scratch. \cite{sam2017arxiv} introduced a switch classifier using VGG-16\cite{simonyan2015iclr} to relay the crowd scene patch to the best CNN column. The switching is very costly and often not correct. While our SaCNN adapts the feature maps from multiple scales and concatenates them to relay each pedestrian to the best scale in the network.

Similar to~\cite{zhang2015cvpr}, we perform a multi-task optimization in SaCNN to regress both the density map and head count. Differently, ours is a multi-scale fully convolutional network and we propose a relative count loss. The scale-adaptive architecture is similar in spirt to~\cite{ronneberger2015miccai,lin2017cvpr} by combining feature maps of multiple layers; but we use the deconvolutional layer~\cite{noh2015iccv} to adapt the network output instead of upsampling and element-wise summation. Our network design with a backbone of single filter size and multi-scale outputs is new in the crowd counting field. Moreover, we have three-fold more contributions referring to Sec.~\ref{Sec:Intro}: (3)-(5).


%\miaojing{I'll move this last three sentences to related work at some point}


%Regressing the density maps is effective in most cases but is not working so well in those scenes with few people (figxx).




